Hierarchical Pretraining on Multimodal Electronic Health Records

Pretraining has proven to be a powerful technique in natural language processing (NLP), exhibiting remarkable success in various NLP downstream tasks. However, in the medical domain, existing pretrained models on electronic health records (EHR) fail to capture the hierarchical nature of EHR data, limiting their generalization capability across diverse downstream tasks using a single pretrained model. To tackle this challenge, this paper introduces a novel, general, and unified pretraining framework called MEDHMP, specifically designed for hierarchically multimodal EHR data. The effectiveness of the proposed MEDHMP is demonstrated through experimental results on eight downstream tasks spanning three levels. Comparisons against eighteen baselines further highlight the efficacy of our approach.

==> sections/experiment.tex <==
\section{Experiment}
In this section, we will introduce the experiment settings including the pre-training settings and the downstream task settings.
\subsection{Dataset and Preprocessing}

Two public EHR datasets, MIMIC-III \footnote{https://physionet.org/content/mimiciii/1.4/} and MIMIC-IV \footnote{https://physionet.org/content/mimiciv/2.2/}, are adopted for the pretraining, while necessary features regarding the extraction of labels in downstream tasks are masked for the fairness of evaluation. We adopt an EHR-oriented preprocessing pipeline called FIDDLE \cite{tang2020democratizing} for feature and label extraction in stay level. Lengths of time series are unified to 48 hours, which is the upper bound of time series-related tasks mentioned in the FIDDLE. Given that MIMIC-III use ICD-9 while MIMIC-IV contains codes in both ICD-9 and ICD-10 styles, we only select admissions with ICD-9 diagnosis codes to avoid potential conflict between different coding standards. Data stats regarding pretraining and downstream tasks are listed in Table.

\begin{table}[]
\tiny
\begin{tabular}{|l|l|l|}
\hline
\multirow{2}{*}{Pretraining}         & \# of Stays in Stay Level Pretraining                  & 100563 \\
                                     & \# of Admissions in Admission Level Pretraining        & 99000  \\ \hline
\multirow{2}{*}{Stay Level Tasks}    & \# of Stays in ARF Prediction                          & 4205   \\
                                     & \# of Stays in Shock Prediction                        & 6190   \\ \hline
Admission Level Tasks                & \# of Admissions in Readmission Prediction             & 33179  \\ \hline
\multirow{4}{*}{Patient Level Tasks} & \# of Patients in Heart Failure Prediction             & 12320  \\
                                     & \# of Patients in COPD Prediction                      & 29256  \\
                                     & \# of Patients in Amnesia Prediction                   & 11928  \\
                                     & \# of Patients in Heart Failure Prediction (MIMIC-III) & 7522       \\ \hline
\end{tabular}
\end{table}


Considering that extreme sparse features can significantly harm computing efficiency and be memory-burdensome, we filter features with frequency lower than 5\%. After the data preprocessing, each timestamp is in the form of a 1318-dimensional sparse vector, while the static tabular data of each patient is represented as a 73-dimensional sparse vector.

An additional EHR dataset TriNetX, containing patients' temporal health record as well as diagnosis and has been widely utilized in health risk prediction, is also adopted for one of the downstream tasks in this study, while others replies on MIMIC-III.

For data extracted from MIMIC-III, We split the downstream datasets following the typical data spliting ratio 8:1:1 for training, validation and testing, respectively. Implementation details regarding experiments such as hardware and hyperparameters can be found in the appendix. 


\subsection{Evaluation}

Following previous work focusing on stay-level task\cite{yang_how_2021}, we adopt Area Under the Receiver Operating Characteristic curve (AUROC) and Area Under the Precision-Recall curve (AUPR) to evaluate the performance of our proposed model. Considering data imbalanced concerns mentioned by \cite{cui2022medskim}, we choose AUPR, F1 and Cohen's Kappa for the evaluation in the selected patient-level task. For the rigorousness, experiments are repeatedly conducted five times and means of evaluation metrics are recorded as the final results. %Evaluation is performed in two patterns listed below:

%\begin{itemize}


%\item \textbf{Uni-modal Evaluation}: In this setting, we combine our pretrained modality-specific encoders with baselines.%, expecting the enhancement caused by the combination.
%\item \textbf{Multi-modal Evaluation}: In this setting, we combine our multimodal pretrained encoder with a MLP block and directly utilize it for downstream prediction. 

%\end{itemize}
%We select stay- and admission-level tasks for the multimodal evaluation, while uni-modal evaluation is performed on the patient level. Tasks and experiment results are respectively introduced in the rest of this section.


\begin{table*}[t]
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|cc|cc||cc}
\hline

\multirow{3}{*}{\textbf{Modalities}} & \multirow{3}{*}{\textbf{Models}}     & \multicolumn{4}{c||}{\textbf{Stay-level}} & \multicolumn{2}{c}{\textbf{Admission-level}} \\\cline{3-8}
& &\multicolumn{2}{c|}{\textbf{ARF}}                                                       & \multicolumn{2}{c||}{\textbf{Shock}}                                                       & \multicolumn{2}{c}{\textbf{Readmission}}                                    \\ \cline{3-8}
&            & \multicolumn{1}{c}{AUROC}  & \multicolumn{1}{c|}{AUPR}  & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c||}{AUPR} & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c}{AUPR}  \\ \hline

\multirow{2}{*}{Clinical Notes} &
ClinicalT5~\cite{lehman2023clinical}             & 50.06                    &  5.92                 &  56.76                   & 13.01        & 50.95   & 4.59                                \\
& ClinicalBERT~\cite{huang2019clinicalbert}    &51.75 &7.60 &44.28 &9.89 &53.96 &4.93 \\ \hline

\multirow{2}{*}{\makecell[l]{Demographics + \\Clinical Features}}
&F-LSTM~\cite{tang2020democratizing}                      & 69.67                    & 10.57                  & 70.28                    & 23.09             & 49.09 &   3.96                             \\
&F-CNN~\cite{tang2020democratizing}                         & 69.61                    & 10.68                  & 69.27                    & 23.51          &50.51 & 4.81                \\\hline
\multirow{9}{*}{\makecell[l]{Demographics\\+ Clinical Features\\ + Clincial Notes \\(+ Codes)}}
&BertLstm~\cite{yang_how_2021}  & 64.90                    & 9.03                  &  70.22                   &  23.32        &63.35 & 7.24                                 \\
&LstmBert~\cite{yang_how_2021}                 &   61.74                      &  9.79                 &  66.31                   &  22.56          &60.67 &6.84                                      \\
    &BertCnn~\cite{yang_how_2021}                     & 67.04                  &  9.49                   & 64.34        & 21.13            &63.07 &7.19                   \\
&CnnBert~\cite{yang_how_2021}                   & 63.38                    & 10.31                   &  66.40                   & 22.46         &61.59 & 7.04                                     \\ 
&BertStar~\cite{yang_how_2021}                &  58.11                   & 6.86                  & 59.24        & 19.58           &61.28 & 6.84                       \\
&StarBert~\cite{yang_how_2021}                &  51.96                   & 5.73                  &  58.89                   & 16.92          &60.67 &6.84                     \\
&BertEncoder~\cite{yang_how_2021}    & 61.30                    & 9.06                  & 52.88                       & 14.66                        &61.94 & 6.82                                 \\
&EncoderBert~\cite{yang_how_2021}         &  62.65                   &  7.44                    &  61.39                   & 18.66          &60.57 &7.00  
\\ 
\rowcolor{red!20}
\cellcolor{white}& \model~(ours)  & \textbf{71.67}                    & \textbf{11.05}                  & \textbf{70.57}                    & \textbf{24.30}           & \textbf{67.77} & \textbf{9.34}                                              \\\hline
\end{tabular}
}
\caption{Comparison over baselines and \model in stay- and admission-level tasks. Note that for readmission prediction where codes are available as input, baselines from \cite{yang_how_2021} are modified to take codes for modality aggregation as well.}\label{tab:multimodal_stay_admission}
\end{table*}

\begin{comment}
    

\begin{table*}[t]\label{tab:multimodal_ICU_stay}
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|ll|ll|ll|ll}
\hline
\multirow{2}{*}{\textbf{Modalities}} & \multirow{2}{*}{\textbf{Models}}     & \multicolumn{2}{c|}{\textbf{ARF}}                                                       & \multicolumn{2}{c|}{\textbf{Shock}}                                                     & \multicolumn{2}{c|}{\textbf{Mortality}}  & \multicolumn{2}{c}{\textbf{Readmission}}                                    \\ \cline{3-10}
&            & \multicolumn{1}{c}{AUROC}  & \multicolumn{1}{c|}{AUPR}  & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c|}{AUPR} & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c|}{AUPR} & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c}{AUPR} \\ \hline

\multirow{2}{*}{Clinical Notes} &
ClinicalT5               & 50.06                    &  5.92                 &  56.76                   & 13.01        &  72.18         & 26.55  & 50.95   & 4.59                                \\
& ClinicalBERT  &51.75 &7.60 &44.28 &9.89 &58.17 &16.42 &53.96 &4.93 \\ \hline

\multirow{2}{*}{\makecell[l]{Demographics + \\Clinical Features}}
&LSTM\cite{tang2020democratizing}                      & 69.67                    & 10.57                  & 70.28                    & 23.09        &  81.55         & \textbf{48.62}      & 49.09 &   3.96                             \\
&CNN\cite{tang2020democratizing}                         & 69.61                    & 10.68                  & 69.27                    & 23.51        & 80.70          & 42.29     &50.51 & 4.81                \\\hline
\multirow{9}{*}{\makecell[l]{Demographics + \\Clinical Features + \\Clincial Notes}}
&BertLstm\cite{yang_how_2021}  & 64.90                    & 9.03                  &  70.22                   &  23.32       &  80.80         & 45.59   &63.35 & 7.24                                 \\
&LstmBert\cite{yang_how_2021}                 &   61.74                      &  9.79                 &  66.31                   &  22.56        &  78.31         &  42.31  &60.67 &6.84                                      \\
    &BertCnn                     & 67.04                  &  9.49                   & 64.34        & 21.13          &  81.12                      & 44.01  &63.07 &7.19                   \\
&CnnBert                   & 63.38                    & 10.31                   &  66.40                   & 22.46        & 77.25          & 36.43  &61.59 & 7.04                                     \\ 
&BertStar                &  58.11                   & 6.86                  & 59.24        & 19.58         &  76.24                      & 36.12  &61.28 & 6.84                       \\
&StarBert                &  51.96                   & 5.73                  &  58.89                   & 16.92        & 76.19          & 34.87  &60.67 &6.84                     \\
&BertEncoder\cite{yang_how_2021}    & 61.30                    & 9.06                  & 52.88                       & 14.66                       &   74.95          & 35.02   &61.94 & 6.82                                 \\
&EncoderBert         &  62.65                   &  7.44                    &  61.39                   & 18.66         & 74.35          & 33.68  &60.57 &7.00                    \\ 
& \model  & \textbf{71.67}                    & \textbf{11.05}                  & \textbf{70.57}                    & \textbf{24.30}        & \textbf{82.06}          & 42.18   & \textbf{67.77} & \textbf{9.34}                                              \\\hline
\end{tabular}
}
\caption{Comparision over baselines and \model in stay-level tasks.}
\end{table*}

    

\begin{table}[t]
\tiny
\centering

%\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|ll|ll|}
\hline
\multirow{2}{*}{\textbf{Modalities}} & \multirow{2}{*}{\textbf{Models}}     & \multicolumn{2}{c|}{\textbf{ARF}}                                                       & \multicolumn{2}{c|}{\textbf{Shock}}                                                                                    \\ \cline{3-6}
&            & \multicolumn{1}{c}{AUROC}  & \multicolumn{1}{c|}{AUPR}  & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c|}{AUPR}  \\ \hline

\multirow{2}{*}{Clinical Notes} &
ClinicalT5               & 50.06                    &  5.92                 &  56.76                   & 13.01                                    \\
& ClinicalBERT &51.75 &7.60 &44.28 &9.89 \\ \hline

\multirow{2}{*}{\makecell[l]{Demographics + \\Clinical Features}}
&F-LSTM                     & 69.67                    & 10.57                  & 70.28                    & 23.09                                      \\
&F-CNN                       & 69.61                    & 10.68                  & 69.27                    & 23.51                       \\\hline
\multirow{9}{*}{\makecell[l]{Demographics + \\Clinical Features + \\Clincial Notes}}
&BertLstm   & 64.90                    & 9.03                  &  70.22                   &  23.32                                   \\
&LstmBert              &   61.74                      &  9.79                 &  66.31                   &  22.56                                        \\
    &BertCnn                     & 67.04                  &  9.49                   & 64.34        & 21.13                           \\
&CnnBert                   & 63.38                    & 10.31                   &  66.40                   & 22.46                                         \\ 
&BertStar                &  58.11                   & 6.86                  & 59.24        & 19.58                               \\
&StarBert                &  51.96                   & 5.73                  &  58.89                   & 16.92                       \\
&BertEncoder    & 61.30                    & 9.06                  & 52.88                       & 14.66                                                    \\
&EncoderBert         &  62.65                   &  7.44                    &  61.39                   & 18.66                         \\ 
& \textbf{\model}  & \textbf{71.67}                    & \textbf{11.05}                  & \textbf{70.57}                    & \textbf{24.30}                                                     \\\hline
\end{tabular}
%}
\caption{Comparision over baselines and {\model} in stay-level tasks.}\label{tab:multimodal_ICU_stay}
\end{table}

\begin{table}[t]
\tiny
\centering

%\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|ll|}
\hline
\multirow{2}{*}{\textbf{Modalities}} & \multirow{2}{*}{\textbf{Models}}     & \multicolumn{2}{c|}{\textbf{Readmission}}                                                                                                  \\ \cline{3-4}
&            & \multicolumn{1}{c}{AUROC}  & \multicolumn{1}{c|}{AUPR}    \\ \hline

\multirow{2}{*}{Clinical Notes} &
ClinicalT5              & 50.95   & 4.59                                \\
& ClinicalBERT   &53.96 &4.93 \\ \hline

\multirow{2}{*}{\makecell[l]{Demographics + \\Clinical Features}}
&F-LSTM                      & 49.09 &   3.96                             \\
&F-CNN                        &50.51 & 4.81                \\\hline
\multirow{9}{*}{\makecell[l]{Demographics + \\Clinical Features + \\Clincial Notes + Codes}}
&BertLstm+  &63.35 & 7.24                                 \\
&LstmBert+                &60.67 &6.84                                      \\
    &BertCnn+                     &63.07 &7.19                   \\
&CnnBert+                   &61.59 & 7.04                                     \\ 
&BertStar+                 &61.28 & 6.84                       \\
&StarBert+                &60.67 &6.84                     \\
&BertEncoder+   &61.94 & 6.82                                 \\
&EncoderBert+          &60.57 &7.00                    \\ 
& \textbf{\model}   & \textbf{67.77} & \textbf{9.34}                                              \\\hline                        
\end{tabular}
%}
\caption{Comparision over baselines and {\model} in admission-level task.}\label{tab:multimodal_admission}
\end{table}

\end{comment}

\subsection{Stay-Level Tasks}

For tasks in stay level, we adopt predictions of two severe clinical illnesses, i.e. ARF and shock, within a 48-hour window. We select multimodal baselines reported in \cite{yang_how_2021} that also adopt modality-specific encoders and perform modality aggregation via gating mechanism. Bimodal models conducting simple modality aggregation in the input stage \cite{tang2020democratizing} are also considered as baselines in our study. Besides, we also select clinical language models \cite{lehman2023clinical, alsentzer2019publicly} for a comprehensive comparison. 

Experiment results are listed in Table \ref{tab:multimodal_stay_admission}. Two unimodal language models, ClinicalT5 and ClinicalBERT, fail to achieve promising performance, which may be attributed to the noisy characteristic of clinical notes. Lightweight bimodal baselines outperform gating-based architectures as the tiny scale of these downstream datasets may impede the usage of complicated models. Our model, benefiting from the pretraining process and acquiring decent suitability in low-resourced setting, manifests competitive performance across multiple stay-level tasks compared with both conventional unimodal baselines, simple bimodal models and advanced multimodality-oriented counterparts. 
\begin{comment}
\begin{itemize}

    \item \textbf{LSTM} is widely accepted for temporal data analysis. Its cell setting enabling the long-dependency capturing allows the model to address sequential tasks in either Monitoring or Patient level. In Monitoring level, it serves as the uni-modal encoder for clinical time series, assisted by a MLP used for processing demographic table .   
    \item \textbf{Transformer} has been utilized in handling sequential data due to its attention mechanism. Similar with LSTM, it is jointly used with a MLP.
    \item \textbf{Raim} is an attention-based model specially designed for analyzing ICU monitoring data, which uses a combination of attention mechanisms and multimodal data integration.
    \item \textbf{DCMN} combines two separate memory networks, one for processing clinical time series and one for processing static table. Its dual-attention mechanism design allows the model to aggregate features effectively.
    \item \textbf{Mufasa} utilize autoML techniques to discover optimal architecture for fusing multiple modalities and conduct health-related tasks. It is designed to be flexiable for different type of EHR data.
\end{itemize}
\end{comment}



\begin{table*}[]
\tiny
\centering
\begin{tabular}{l|ll|ll|ll|}
                         & \multicolumn{2}{c|}{ARF}                                                       & \multicolumn{2}{c|}{Shock}                                                     & \multicolumn{2}{c|}{Mortality}                                      \\ \hline
                        & \multicolumn{1}{c}{AUROC}  & \multicolumn{1}{c|}{AUPR}  & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c|}{AUPR} & \multicolumn{1}{c}{AUROC} & \multicolumn{1}{c|}{AUPR}  \\ \hline
                                
LSTM(w. hierarchical pt)        &  \textbf{57.40}                   &  \textbf{6.99}                 & \textbf{61.76}                    & \textbf{16.36}        &  \textbf{76.57}         &  30.91                         \\
LSTM(w. uni-level pt)           &  55.74                   &  6.93                 &  58.93                   & 16.34        &  75.93         & \textbf{32.69}                        \\
LSTM(w/o pt)                  &     55.25                 & 6.37                  & 57.88                    & 16.01          &   74.41        &  29.99                               \\ \hline
Transformer(w. hierarchical pt) &   \textbf{59.11}                  &   \textbf{7.12}                & \textbf{63.47}                    & \textbf{18.35}        &  \textbf{76.73}         &  \textbf{36.70}                           \\
Transformer(w. uni-level pt)    &   58.01                  &   7.10                &  61.65                   & 17.72        &  75.58         &  32.29                            \\
Transformer(w/o pt)              &  55.48                   &  7.09                &    61.87                 & 15.67        &  72.21         &  33.79                              \\ \hline
\end{tabular}
\label{Unimodal encoder}
\caption{Comparison over Baselines with/without Pretrained Layers on ICU Level Task.}
\end{table*}





\begin{comment}
    

\begin{table}[]
\begin{tabular}{l|lll|lll|lll|}
                                & \multicolumn{3}{c|}{ARF}                       & \multicolumn{3}{c|}{Shock}                     & \multicolumn{3}{c|}{Mortality}                   \\
                                \hline
                                & AUPR           & F1            & Kappa         & AUPR           & F1            & Kappa         & AUPR           & F1             & Kappa          \\ \hline
LSTM(w. hierarchical pt)        & 8.42           & \textbf{2.10} & 1.42             & 22.10          & 9.46          & 6.42          & 39.36          & 35.89          & 29.30          \\
LSTM(w. uni-level pt)           & \textbf{10.31} & 4.12          & \textbf{1.35} & \textbf{22.61} & \textbf{7.04} & \textbf{5.01} & \textbf{42.31} & \textbf{36.72} & \textbf{29.62} \\
LSTM(w/o pt)                   & 8.36                     & 0                   & 0          & 20.00          & 3.24          & 2.46          & 41.26          & 31.18          & 25.25          \\ \hline
Transformer(w. hierarchical pt) & \textbf{10.09} & \textbf{9.55} & \textbf{5.61} & \textbf{26.07} & \textbf{6.80} & \textbf{5.95} & 40.50          & \textbf{40.70} & \textbf{32.27} \\
Transformer(w. uni-level pt)    & 9.84           & 3.75          & 1.00          & 22.82          & 2.27          & 2.58          & \textbf{41.75} & 40.38          & 31.53          \\
Transformer(w/o pt)              & 9.15                     & 5.49                   & 3.42          & 21.78          & 2.98          & 2.55          & 41.67          & 36.03          & 29.11          \\ \hline
\end{tabular}
\label{Unimodal encoder}
\caption{Comparison over Baselines with/without Pretrained Layers.}
\end{table}






\begin{table}[]
\begin{tabular}{l|lll|lll|lll|}
                         & \multicolumn{3}{c|}{ARF}                                                       & \multicolumn{3}{c|}{Shock}                                                     & \multicolumn{3}{c|}{Mortality}                                                 \\ \hline
                         & \multicolumn{1}{c}{AUPR} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{Kappa} & \multicolumn{1}{c}{AUPR} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{Kappa} & \multicolumn{1}{c}{AUPR} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{Kappa} \\ \hline
LSTM                     & 8.36                     & 0                   & 0                       & 22.32                    & 3.00                   & 2.49                       & 41.26                    & 31.18                  & 25.25                      \\
Transformer              & 9.15                     & 5.49                   & 3.42                       & 21.78                    & 2.98                   & 2.55                       & 41.67                    & 36.03                  & 29.11                      \\
Raim                     & 11.04                    & 12.93                  & 6.69                      & 20.90                    & 13.82                  & 9.66                       & 42.14                    & 37.98                  & 31.32                      \\
DSMN                     & 11.19                    & 9.20                  & 4.82                       & 16.88                    & 14.08                  & 6.09                       & 42.30                    & 40.29                  & 33.67                      \\
Mufasa                   & 12.35                    & 7.20                   & 5.56                       & 16.54                    & 6.38                   & 2.97                       & 36.51                    & 33.80                  & 26.11                      \\ \hline
HMMP(w. hierarchical pt) & \textbf{13.16}                    & \textbf{11.42}         & \textbf{9.46}             & \textbf{23.47}           & 10.68                  & 7.11                       & 45.46                    & \textbf{41.58}         & 34.64                      \\
HMMP(w. uni-level pt)    & 11.02                    & 4.09                   & 2.45                       & 22.65                    & \textbf{14.88}         & \textbf{10.43}             & 42.37                    & 36.56                  & 29.50                      \\
HMMP(w/o pt)             & 13.04           & 11.21                   & 8.43                       & 21.20                    & 11.11                  & 7.64                       & \textbf{47.12}           & 41.07                  & \textbf{34.82}             \\ \hline
\end{tabular}
\label{Multimodal encoder}
\end{table}

\end{comment}












\subsection{Admission-Level Task}

 Besides stay-level tasks mentioned above, we also adopt the task, readmission prediction within 30 days, as the representative of tasks in the admission level, where diagnosis and drug codes are available as input of models. For the fair comparison, we assign baselines introduced in \cite{yang_how_2021} with these modalities as additional input, such that {\model} and these baselines share the same inputs. Following the original design, these inputs are embedded through linear layers and aggregated using the gating module. For the same consideration, we perform pooling operation on latent representation of multiple clinical time series belonging to a specific admission, such that baselines can also take advantages from multiple stays. 
 
 Experimental results of readmission predction are listed in Table \ref{tab:multimodal_stay_admission}. It is observed that unimodal language models and simple bimodal baselines expose insufficient capability on handling task in this level, indicating the necessity of introducing additional information from more modalities. Compared with complicated baselines in \cite{yang_how_2021}, {\model} takes a further step on learning from the pretraining stage and thus manifest competitive performance.   
\begin{comment}
    

 \begin{table}[t]
\tiny
\centering
\begin{tabular}{l|lll|}

                         & \multicolumn{1}{c}{AUPR} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c|}{Kappa} \\ \hline
                                
ClinicalBert\cite{alsentzer2019publicly}        &                     &                   &                             \\
ClinicalT5\cite{lehman2023clinical}           &                     &                   &                      \\ \hline
A + B1 + C + D\cite{sheetrit2023predicting}                 &                     &                   &         \\ 
MedM-PLM \cite{liu2022multimodal}(\xiaochen{Try to see if we can reproduce it..})   &                     &                   &    \\    \hline
\model(w. hierarchical pt)&                     &                   &    \\
\model(w. uni-level pt)    &                     &                   &    \\
\model(w/o pt)             &                     &                   &           \\ \hline
\end{tabular}
\label{Readmission}
\caption{Readmission Prediction Using Different Modalities and Models. Adding pretrained embedding layers is proven to be effective.}
\end{table}
\end{comment}


\begin{table*}[t]
\centering
%\begin{tabular}{|l{H}|lll|lll|lll|lll|lll|}
\resizebox{1\textwidth}{!}{
\begin{tabular}{|l|lll|lll|lll|lll|lll|}
\hline
\textbf{}       & \multicolumn{3}{c|}{Heart Failure}      & \multicolumn{3}{c|}{COPD}                                          & \multicolumn{3}{c|}{Amnesia}    & \multicolumn{3}{c|}{MIMIC-III}                 \\ \hline%
                & AUPR          & F1             & KAPPA          & AUPR          & F1             & KAPPA                 & AUPR          & F1             & KAPPA    & AUPR          & F1             & KAPPA        \\ \hline
HiTANet(w. pt)     & \textbf{60.12} & \textbf{50.48} & \textbf{36.08} &   \textbf{64.04}             &  \textbf{54.46}              &  \textbf{43.38}                          & \textbf{67.54} & \textbf{58.18} & \textbf{47.78} &69.42  &\textbf{68.44}  &\textbf{50.01}\\
HiTANet(w/o pt)    & 54.76          & 47.92          & 32.04          &  60.10              &   52.40             &  39.93                  & 63.08          & 54.60          & 43.44         &\textbf{70.36}  &66.60  &46.60 \\ \hline
LSTM(w. pt)     & \textbf{50.16} & \textbf{46.08} & \textbf{29.26} & \textbf{50.16}          & \textbf{49.34} & \textbf{34.64}             & \textbf{48.68} & \textbf{49.64} & \textbf{34.46} &\textbf{57.83}  &\textbf{59.40}  &\textbf{35.86}\\
LSTM(w/o pt)    & 48.20          & 44.44         & 26.64          & 49.52 & 47.76          & 33.44                     & 47.92          & 48.80          & 32.98         &\textbf{57.83}  &56.70  &33.03 \\ \hline
AdaCare(w. pt)  & \textbf{57.63} & \textbf{47.98} & \textbf{32.03} & 54.06 & \textbf{47.10} & \textbf{34.70}          & \textbf{62.62} & \textbf{52.56} & \textbf{41.54} &58.40  &\textbf{59.47}  &\textbf{35.77}\\
AdaCare(w/o pt) & 55.43          & 45.13          & 31.43          & \textbf{56.63}          & 46.60          & 34.53           & 61.62          & 50.54          & 39.22     &\textbf{59.40}  &57.58  &35.84     \\ \hline
Dipole(w. pt)  &\textbf{47.70}  &\textbf{41.86}  &\textbf{25.52}  &48.92  &\textbf{41.06}  &\textbf{28.30}           & \textbf{48.74} & \textbf{45.78} &\textbf{30.78} &\textbf{59.71}  &\textbf{60.50}  &\textbf{37.68} \\
Dipole(w/o pt)  &47.16  &40.16  &24.28  &\textbf{49.44}  &39.48  &27.86           &48.36  &45.63  &30.40  &59.43  &58.63  &36.03\\ \hline
Retain(w. pt)  &\textbf{58.16}  &\textbf{52.18}  &\textbf{35.64}  & \textbf{57.62} & \textbf{50.66} & \textbf{38.36}          &\textbf{62.70}  &\textbf{56.50}  &\textbf{43.90} &\textbf{68.71}  &\textbf{66.20}  &\textbf{47.12} \\
Retain(w/o pt)  &57.50  &50.88  &34.52  & 57.40 & 49.85 & 37.36          &62.52  &56.32  &43.66  &67.76  &65.56  &45.63\\ \hline

\end{tabular}
}
\caption{\centering Health risk prediction with/without pretraining. Comparisons across different datasets and baselines show the model-agnostic boosting brought by pretraining. }\label{Health Risk Prediction}
\end{table*}
 
 \subsection{Patient Level Task}
 \subsubsection{Unimodal Encoder Evaluation}
Even though {\model} has not been pretrained on patient-level tasks, it is still capable of handling tasks in this level since its unimodal encoders acquire the ability of generating high-quality representation of each admission, thus become feasible to be utilized to boost existing time series-targeting models. we Health risk prediction, which utilizes sequence of hospital admissions for illness forecasting, is applied as the task in the patient level. Following deep learning architectures are chosen as the baselines in this level:

\begin{itemize}
    \item \textbf{LSTM}\cite{hochreiter1997long} is a typical backbone model appearing in time series forecasting tasks.
    \item \textbf{HiTANet}\cite{luo2020hitanet} adopts the time-aware attention mechanism design that enables itself to capture the dynamic disease progression pattern.
    \item \textbf{Dipole}\cite{ma2017dipole} relies on the combination of bidirectional GRU and attention mechanism to analyze sequential visits of a patient. 
    \item \textbf{AdaCare}\cite{ma2020adacare} applies the Convolutional Neural Network for feature extraction, followed by a GRU block for prediction.
    \item \textbf{Retain} \cite{choi2016retain} utilizes reverse time attention mechanism to capture dependency between various visits of a patient.
\end{itemize}

Originally, these baselines take series of diagnosis codes as input. In our experiments, the pretrained diagnosis code encoder is applied to baselines for projecting codes to the pretrained latent space. To eliminate irrelevant variables, baselines are using the same set of hyperparameters regardless of whether pretrained encoders are used.

Results in Table \ref{Health Risk Prediction} show the improvement introduced by the addition of hierarchically pretrained unimodal encoder, not only revealing the effectiveness of {\model} in patient level task but also signifying the model-agnosticity of {\model}, indicating its wide range of application in diverse medical scenarios regardless of which combination of modalities are covered in the application.





%\begin{itemize}


%\item \textbf{Acute kidney failure (ARF) prediction}: ARF is a clinical problem frequently occurring in the ICU, whose associated mortality is between 50\% and 80\%. 
%\item \textbf{Shock prediction}: Shock refers to a state of organ hypoperfusion that may result in organ failure or even death. 
%\item \textbf{Mortality prediction}: In this task, the model is responsible to predict whether the patient will die given a 48-hours long window of ICU monitoring data.

%\end{itemize}



%\begin{itemize}

%\item \textbf{Health risk prediction}: Health risk prediction aims at predicting the likelihood of an individual developing a specific disease or health condition in the future, given the previous clinical record of this patient.  
%\item \textbf{Readmission prediction}: Readmission prediction focuses on predicting whether a patient who has been discharged from a hospital will be readmitted within a specific time frame. In the experiment setting of our work, we specifically consider the prediction on whether the readmission will occur within 30 days after the discharging, which is decided based on the medicare reimbursement policy.

%\end{itemize}














\begin{comment}
    

\begin{table}[]
\footnotesize
\begin{tabular}{lllllll}
            & \multicolumn{2}{l}{ARF} & \multicolumn{2}{l}{Shock} & \multicolumn{2}{l}{Mortality} \\
            \hline
            & AUROC        & AUPR        & AUROC          & AUPR         & AUROC            & AUPR           \\
            \hline
LSTM        & 64.04      & 11.67      & 65.02       & 19.04       & 79.45         & 35.93         \\

Transformer & 70.57      & 13.99      & 65.55       & 18.80       & \textbf{82.79}        & 42.47         \\

Raim        & 59.35      & 7.11      & 65.49       & 20.99       & 78.43         & 37.04        \\

DCMN   & 62.54      & 9.32      & 71.15       & 24.89       & 80.96         & 41.97        \\

Mufasa & 69.98      & 11.36      & 67.71       & 21.95       & 76.62         & 32.26       \\
\hline
HMMP(double pt)        & 69.68      & 17.15      & \textbf{72.67}       & \textbf{31.91}       & 82.04         & 48.52        \\

HMMP(icu pt)   & \textbf{70.93}      & 15.06      & 72.45      & 29.49       & 82.39         & 46.79        \\

HMMP(w/o pt)& 69.03      & \textbf{18.69}      & 72.57      & 29.52      & 81.91         & \textbf{48.85}       \\
\hline

\end{tabular}
\caption{Comparison over Baselines and Multimodal Encoder with/without Pretrained Layers}
\end{table}
\end{comment}




\begin{comment}
\begin{table}[]
\footnotesize
\begin{tabular}{lllllll}
            & \multicolumn{2}{l}{ARF} & \multicolumn{2}{l}{Shock} & \multicolumn{2}{l}{Mortality} \\
            \hline
            & AUROC        & AUPR        & AUROC          & AUPR         & AUROC            & AUPR           \\
            \hline
LSTM(double pt)        & \textbf{66.57}      & 10.07      & \textbf{68.36}       & 20.18       & 79.27         & 36.60        \\

LSTM(icu pt)   & 64.40      & \textbf{13.63}      & 67.02       & \textbf{20.51}       & \textbf{80.78}         & \textbf{38.29}      \\

LSTM(w/o pt)& 64.04      & 11.67      & 65.02       & 19.04      & 79.45         & 35.93       \\
\hline
Transformer(double pt)        & \textbf{70.86}      & 13.99      & 65.81       & \textbf{20.52}       & \textbf{82.85}        & 42.16        \\

Transformer(icu pt)   & 70.85      & \textbf{17.27}      & \textbf{66.63}       & 19.79       & 82.62         & \textbf{44.42}        \\

Transformer(w/o pt)& 70.57      & 13.99       &65.55       & 18.80       & 82.79         & 42.47       \\
\hline

\end{tabular}
\caption{Comparison over Baselines with/without Pretrained Layers}
\end{table}
\end{comment}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}



%\begin{table}[]
%\tiny
%\begin{tabular}{|l|lll|lll|lll|lll|lll|}
%\hline
%\textbf{}       & \multicolumn{3}{c|}{\textbf{Heart Failure}}      & \multicolumn{3}{c|}{COPD}                        & \multicolumn{3}{c|}{Kidney}                      & \multicolumn{3}{c|}%{Dementia}                    & \multicolumn{3}{c|}{Amnesia}                     \\ \cline{2-16} 
%                & PRAUC          & F1             & KAPPA          & PRAUC          & F1             & KAPPA          & PRAUC          & F1             & KAPPA          & PRAUC          & F1  %           & KAPPA          & PRAUC          & F1             & KAPPA          \\ \hline
%HITA(w. pt)     & \textbf{65.26} & \textbf{60.00} & \textbf{44.72} &   \textbf{67.50}             &  \textbf{60.80}              &  47.46              &      TBP          &       TBP         &    TBP            &  \textbf{50.63}              &  \textbf{48.58}             &   \textbf{33.13}             & \textbf{68.42} & \textbf{61.80} & \textbf{50.40} \\
%HITA(w/o pt)    & 63.80          & 56.94          & 41.46          &  67.08              &   60.16             &  \textbf{47.54}              &   TBP             &    TBP            &    TBP            &  49.48              &  48.08              &   32.63             & 67.78          & 61.56          & 49.30          \\ \hline
%LSAN(w. pt)     & 52.54          & 40.76          & 27.30          & \textbf{58.72} & \textbf{52.24} & \textbf{39.10} & 63.68          & 56.84          & 44.58          & \textbf{43.02} & \textbf{34.05} & \textbf{21.35} & 58.98          & 53.20          & 41.92          \\
%LSAN(w/o pt)    & \textbf{53.56} & \textbf{42.86} & \textbf{29.32} & 58.16          & 51.36          & 38.44          & \textbf{67.58} & \textbf{60.62} & \textbf{48.60} & 42.50          & 30.06          & 18.26          & \textbf{62.52} & \textbf{56.82} & \textbf{45.04} \\ \hline
%LSTM(w. pt)     & \textbf{49.62} & \textbf{55.64} & \textbf{38.40} & 50.90          & \textbf{52.12} & \textbf{37.12} & \textbf{56.70} & \textbf{61.90} & \textbf{47.26} &   46.46             &   41.87             &   \textbf{29.00}             & \textbf{51.38} & \textbf{57.72} & \textbf{42.50} \\
%LSTM(w/o pt)    & 48.24          & 55.50          & 37.50          & \textbf{51.34} & 51.60          & 36.96          & 55.24          & 61.86          & 47.24          &  \textbf{46.68}              &     \textbf{41.95}           &   28.68             & 48.22          & 57.04          & 41.70          \\ \hline
%AdaCare(w. pt)  & \textbf{52.80} & \textbf{54.44} & \textbf{37.44} & \textbf{57.05} & \textbf{53.55} & \textbf{41.00} & \textbf{58.88} & 59.86          & 45.18          & \textbf{49.56} & \textbf{49.08} & 32.12          & \textbf{61.04} & \textbf{57.16} & \textbf{45.04} \\
%AdaCare(w/o pt) & 51.84          & 53.02          & 36.36          & 57.00          & 53.16          & 40.20          & \textbf{58.88} & \textbf{60.36} & \textbf{46.16} & 49.26          & 48.68          & \textbf{33.86} & 57.06          & 55.90          & 42.64          \\ \hline
%\end{tabular}
%\end{table}
\begin{comment}
\begin{table}[]
\tiny
\centering
\begin{tabular}{|l|lll|lll|lll|lll|lll|}
\hline
\textbf{}       & \multicolumn{3}{c|}{Heart Failure}      & \multicolumn{3}{c|}{COPD}                        & \multicolumn{3}{c|}{Kidney}                      & \multicolumn{3}{c|}{Dementia}                    & \multicolumn{3}{c|}{Amnesia}                     \\ \cline{2-16} 
                & AUPR          & F1             & KAPPA          & AUPR          & F1             & KAPPA          & AUPR          & F1             & KAPPA          & AUPR          & F1             & KAPPA          & AUPR          & F1             & KAPPA          \\ \hline
HITA(w. pt)     & \textbf{65.26} & \textbf{60.00} & \textbf{44.72} &   \textbf{67.50}             &  \textbf{60.80}              &  47.46              &      \textbf{49.78}          &       \textbf{48.06}        &    \textbf{32.20}            &  \textbf{50.63}              &  \textbf{48.58}             &   \textbf{33.13}             & \textbf{68.42} & \textbf{61.80} & \textbf{50.40} \\
HITA(w/o pt)    & 63.80          & 56.94          & 41.46          &  67.08              &   60.16             &  \textbf{47.54}              &   49.22             &    47.22            &    31.96            &  49.48              &  48.08              &   32.63             & 67.78          & 61.56          & 49.30          \\ \hline
LSTM(w. pt)     & \textbf{49.62} & \textbf{55.64} & \textbf{38.40} & 50.90          & \textbf{52.12} & \textbf{37.12} & \textbf{56.70} & \textbf{61.90} & \textbf{47.26} &   46.46             &   41.87             &   \textbf{29.00}             & \textbf{51.38} & \textbf{57.72} & \textbf{42.50} \\
LSTM(w/o pt)    & 48.24          & 55.50          & 37.50          & \textbf{51.34} & 51.60          & 36.96          & 55.24          & 61.86          & 47.24          &  \textbf{46.68}              &     \textbf{41.95}           &   28.68             & 48.22          & 57.04          & 41.70          \\ \hline
AdaCare(w. pt)  & \textbf{52.80} & \textbf{54.44} & \textbf{37.44} & \textbf{57.05} & \textbf{53.55} & \textbf{41.00} & \textbf{58.88} & 59.86          & 45.18          & \textbf{49.56} & \textbf{49.08} & 32.12          & \textbf{61.04} & \textbf{57.16} & \textbf{45.04} \\
AdaCare(w/o pt) & 51.84          & 53.02          & 36.36          & 57.00          & 53.16          & 40.20          & \textbf{58.88} & \textbf{60.36} & \textbf{46.16} & 49.26          & 48.68          & \textbf{33.86} & 57.06          & 55.90          & 42.64          \\ \hline
%Retain(w. pt)  & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} & TBP          & TBP          & \textbf{TBP} & \textbf{TBP} & TBP         & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} \\
%Retain(w/o pt) & TBP         & TBP        & TBP        & TBP         & TBP         & TBP          & \textbf{TBP} & \textbf{TBP} & \textbf{TBP} & TBP          & TBP         & \textbf{TBP} &TBP        & TBP          & TBP          \\ \hline
Dipole(w. pt)  & \textbf{47.20} & \textbf{54.24} & 36.02 & \textbf{52.24} & 51.68 & \textbf{36.98} & 50.56 & \textbf{61.00}         & \textbf{45.94}          & \textbf{48.26} & \textbf{47.64} & \textbf{31.22}         & \textbf{55.40} & \textbf{57.08} & \textbf{45.26} \\
Dipole(w/o pt) & 46.94        & 53.88       & \textbf{36.42}          & 52.18       & \textbf{51.82}       & 36.96         & \textbf{51.26} & 60.58 & 45.42 & 48.22         & 47.22         &  30.92 & 53.14        & 56.66       & 44.28          \\ \hline


\end{tabular}

\caption{\centering Health risk prediction with/without pretraining. Comparisons across different datasets and baselines show the model-agnostic boosting brought by pretraining.}
\end{table}

\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\begin{table}[]
\tiny
\centering
%\begin{tabular}{|l{H}|lll|lll|lll|lll|lll|}
\begin{tabular}{|l|lll|lll|lll|lll|lll|}
\hline
\textbf{}       & \multicolumn{3}{c|}{Heart Failure}      & \multicolumn{3}{c|}{COPD}                                          & \multicolumn{3}{c|}{Amnesia}                     \\ \hline%\cline{2-16} 
                & AUPR          & F1             & KAPPA          & AUPR          & F1             & KAPPA                 & AUPR          & F1             & KAPPA          \\ \hline
HITA(w. pt)     & \textbf{65.26} & \textbf{60.00} & \textbf{44.72} &   \textbf{67.50}             &  \textbf{60.80}              &  47.46                          & \textbf{68.42} & \textbf{61.80} & \textbf{50.40} \\
HITA(w/o pt)    & 63.80          & 56.94          & 41.46          &  67.08              &   60.16             &  \textbf{47.54}                  & 67.78          & 61.56          & 49.30          \\ \hline
LSTM(w. pt)     & \textbf{49.62} & \textbf{55.64} & \textbf{38.40} & 50.90          & \textbf{52.12} & \textbf{37.12}             & \textbf{51.38} & \textbf{57.72} & \textbf{42.50} \\
LSTM(w/o pt)    & 48.24          & 55.50          & 37.50          & \textbf{51.34} & 51.60          & 36.96                     & 48.22          & 57.04          & 41.70          \\ \hline
AdaCare(w. pt)  & \textbf{52.80} & \textbf{54.44} & \textbf{37.44} & \textbf{57.05} & \textbf{53.55} & \textbf{41.00}          & \textbf{61.04} & \textbf{57.16} & \textbf{45.04} \\
AdaCare(w/o pt) & 51.84          & 53.02          & 36.36          & 57.00          & 53.16          & 40.20           & 57.06          & 55.90          & 42.64          \\ \hline
Dipole(w. pt)  & \textbf{47.20} & \textbf{54.24} & 36.02 & \textbf{52.24} & 51.68 & \textbf{36.98}          & \textbf{55.40} & \textbf{57.08} & \textbf{45.26} \\
Dipole(w/o pt) & 46.94        & 53.88       & \textbf{36.42}          & 52.18       & \textbf{51.82}       & 36.96          & 53.14        & 56.66       & 44.28          \\ \hline


\end{tabular}
\label{Health Risk Prediction}
\caption{\centering Health risk prediction with/without pretraining. Comparisons across different datasets and baselines show the model-agnostic boosting brought by pretraining. }
\end{table}
\end{comment}


%\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}


==> sections/initialization.tex <==
%\section{Initialization}

\paragraph{Data-wise Initialization Test}
Intuitively, pretraining could result in better initialization performance compared with models trained from scratch, enhancing its suitability in low-resourced setting such as zero-shot learning and few-shot learning. Inspired by this characteristics, we explore the low-resourced setting that simulate common real-world health-related scenario, in which dataset curation demands professional knowledge. In these experiment, we reconduct experiments introduced in the previous section, but with shrinking dataset. For a hyperparameter $k$ indicating the proportion of data used in training, we select $k\%$ of the original data for training, and change the value of $k$ to explore the relation between the volume of training data and performance. For each $k$, we perform the training on the same model with/without pretraining, to investigate their adaptability in low-resourced setting contrastively. The visualization in Figure~\ref{Fig.init1} below demonstrates how the performance of model shift as the amount of training data changes. 



\begin{figure}[t!]
\centering  
\subfigure[Amnesia Prediction with HiTANet]{
\label{Fig.sub.2}
\includegraphics[width=0.46\textwidth]{fig/health_risk_proportion_1.pdf}}
 \subfigure[Amnesia Prediction with LSTM]{
\label{Fig.sub.1}
 \includegraphics[width=0.46\textwidth]{fig/health_risk_proportion_2.pdf}}
% \subfigure[A-CRF]{
% \label{Fig.sub.3}
% \includegraphics[width=0.4\textwidth]{fig/A_CRF.pdf}}
% \subfigure[C-CRF]{
% \label{Fig.sub.4}
% \includegraphics[width=0.4\textwidth]{fig/C_CRF.pdf}}


\caption{This figure shows how performance shifts according to proportion of data used in training. Comparison between these two curses shows that the pretraining enables model to be more competitive in the initialization.}
\label{Fig.init1}
\end{figure}

According to the experiment results, the hierarchical pretraining is capable of initializing the target model regardless of tasks, levels as well as involved modalities, exactly addressing the general concern frustrating researchers in the domain of health informatics. 


\paragraph{Epoch-wise Initialization Test}

\begin{figure}[t!]
\centering  
\subfigure[Heart Failure Prediction with LSTM]{
\label{Fig.sub.2}
\includegraphics[width=0.46\textwidth]{fig/init_epoch_1.pdf}}
 \subfigure[COPD Prediction with HiTANet]{
\label{Fig.sub.1}
 \includegraphics[width=0.46\textwidth]{fig/init_epoch_2.pdf}}
% \subfigure[A-CRF]{
% \label{Fig.sub.3}
% \includegraphics[width=0.4\textwidth]{fig/A_CRF.pdf}}
% \subfigure[C-CRF]{
% \label{Fig.sub.4}
% \includegraphics[width=0.4\textwidth]{fig/C_CRF.pdf}}


\caption{Placeholder for epoch-wise initialization test.}
\label{Fig.init2}
\end{figure}

Similarly, if the excellent initialization is proven to help models converge to better results with less amount of data, it can also assist the model to achieve decent performance while spending less time on converging. Therefore, we conduct the epoch-wise experiments to further illustrate how our pretraining strategy alleviates the time-consuming problem, stating that our model is not only effective but also efficient, in a generalization perspective.




==> sections/introduction.tex <==
\section{Introduction}
%%\subsection{Background and Related Work}

%Pretraining has been commonly perceived as effective method for digging  

Along with the increasing availability of Electronic Health Records (EHRs), researchers in the field of health informatics have attempted to utilize EHR to develop specific models automatically handling healthcare-related tasks for years. However, the heterogeneous nature of EHRs, which is partially but not thoroughly discussed by previous works \cite{pivovarov2015learning, rasmy2018study}, notably affects the utilization of abundant information contained in this complex form of data. In recent years, researchers have started to investigate the potential of utilizing multimodal learning to solve health-related problems, marking the march to aggregate heterogeneous features. However, the heterogeneity introduced by the hierarchy of EHRs determining which part of data should be used as input given a specific task is understudied and occasionally neglected. For instance, for predicting illness such as Acute Renal Failure (ARF) extracted from lab test record that is only associated with each Intensive Care Unit (ICU) stay, previous work \cite{yang_how_2021} utilizes discharge summary corresponding to each visit to hospital that can cover multiple ICU stays. This type of ill-aligned relation between input and prediction target can result in problematic application in real-world setting since discharge summary can never be obtained while medical practitioners struggling in ICU are eager for the risk possibility, demonstrating the necessity of rethinking the heterogeneous nature in the hierarchy of EHRs, and propose analysis and solution accordingly. 

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{fig/data_structure.pdf}
\caption{An illustration of EHR hierarchy.
\vspace{-.1in}
}
\label{fig:data}
\end{figure*}

%\xiaochen{Deep learning models' capability on feature extraction and performance boosting makes it a more ideal choice compared to conventional machine learning models highly relying on hand-crafted features as well as manually injected external knowledge.}

%In MIMIC-III and MIMIC-IV \footnote{https://physionet.org/content/mimiciii/1.4/} \footnote{https://physionet.org/content/mimiciv/2.2/} that serve as the data resources in this study, data can be categorized into three granlarities: 

From bottom to top, granlarities in EHR data can be defined as listed below : 


\begin{itemize}
    \item \textbf{Monitoring stays} refers to the period in which a patient is monitored in ICU. Data relevant to this period are collected through multiple sources such as input and output record of patient, monitoring devices deployed in ICU, etc.
    \item \textbf{Hospital admission} refers to a specific period of hospitalization. Each hospital admission may contain any number of monitoring stays. In some cases, a patient can visit hospital without any time staying at ICU. 
    \item \textbf{Patient} includes all information regarding a specific patient. Each patient may have single or multiple hospital admission to hospital according to the EHRs.


\end{itemize}

Some health-related tasks are listed in \ref{Granularity}, along with granularities they belong to. This table provide an impression of how data and tasks manifest heterogeneity in a vertical perspective, deepen the complexity of EHRs datasets after combining with its multi-modal nature that divide data in a horizontal dimension.

%Pretraining has been perceived as a solution to allevate the heterogeneity problem in several domains such as natural language processing \cite{liu2022oag} and graph

Multimodal pretraining has been perceived as a solution aggregating different tasks and heterogeneous data. Previous works try to aggregate distinct modalities to produce a model capable of handing multi-tasks, which matches the challenge in EHRs data exactly. In the field of health informatics, researchers have paid special attention to the pretraining on clinical notes considering the rich information it convey. However, most of these effort only consider utilize two modalities instead of more of them \cite{park_graph-text_2022, plasser2022multimodal}, limiting their applications in a wider range of tasks. For instance, a model pretrained merely using discharge summary and its corresponding graph representation cannot be utilized in ARF prediction due to ill-aligned problem mentioned above, thus emphasizing the importance of conducing pretraining involving more modalities across different level in EHR hierarchy.

Therefore, we propose the \model to address all the concerns discussed and analyzed. In the design of \model, we take care of four modalities in total: clinical time series, demographic table, ICD diagnosis code and pharmaceutical code, which can cover tasks among all three granularities listed in \ref{Granularity}. The hierarchical factor neglected by most of works is taken into consideration in the pretraining strategy, resulting in the hierarchical pretraining that accurately match domain-specific downstream tasks. Experiments show that our proposed \model  is effective and can be utilized to boost performance of other models through the enhancement of medical representation. Further studies show that models with boosting from \model can be equipped with a better capability of initialization, which is more than significant in medical applications in which low-resourced setting is popular. 











\begin{table}[]
\centering
\begin{tabular}{|l|l|}

\hline
Task                            & Granularity \\ \hline
Mortality Prediction            & Monitoring        \\
Acute Kidney Failure Prediction & Monitoring        \\
Shock Prediction                & Monitoring        \\
Readmission Prediction          & Hospitalization        \\
Health Risk Prediction          & Patient     \\\hline
\end{tabular}
\caption{Correspondence between tasks and granularities that they are in.}
\label{Granularity}
\end{table}

==> sections/limitations.tex <==
\section{Limitations}

% The experiments regarding multimodal encoder demonstrate competitive performance, showing the reasonability of our pretraining architecture design. Besides, unimodal encoders for respective modality manifest model-agnostic and task-agnostic through the comparison conducted across diverse downstream baselines and tasks.

% However, it is also worth mentioning that the boosting is not very stable in some of scenarios, discussion of whom may be as valuable as the proposed method. Different from pretraining in general domain, the pretraining on EHR data suffers from the dilemma prevalent in the field of healthcare, which is the limitation of data volume. Even though external data are introduced from MIMIC-IV to boost the downstream tasks, it is notable that the additional resources is still not sufficient enough compared to pretraining in the domain of NLP or CV, in which millions of clean and well-organized data are accessible. We believe that this problem will be resolved as long as more EHRs become available.

% One may ask why natural language is not utilized in the pretraining stage in this work, since it is widely acknowledged that encoders of existing large language model (LLM) can be directly adopted to generate text representation in high-quality. An unimodal encoder pretrained on clinical domain such as Clinical BERT hold the potential of being jointly used along with other modalities to further boost the quality of EHR representation. This conceive is prohibited by the incompletedness of MIMIC-IV dataset, as the part of clinical notes has not been fulfilled. We hold it firmly that adding natural language to our current architecture can be beneficial and will be feasible once the expected data become accessible. 

==> sections/methodology.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.1\textwidth]{fig/model_draft.pdf}
\caption{A demo of model illustration. Further improvement needed. 
\vspace{-.1in}
}
\label{fig:model}
\end{figure}

\section{Methodology}

%Considering that EHR data are in diverse granularities including patient, HADM (visit) and ICU stay, the hierarchy cannot be simply tackled by a single model. To address this difficulty, we design the Hierarchical MultiModal Pretraining framework to complete the pretraining task in a bottom-to-up pattern, obtaining representation of EHR data in each possible granularity, and enhancing the model's capability of handling downstream tasks in multiple scenarios.


To address the heterogeneity in EHRs, we propose the Hierarchical Multimodal Pretraining framework called \model , leveraging pertraining strategies across different modalities and levels within the EHRs hierarchy for the unification. The pretraining will be conducted in two levels of the hierarchy: ICU stay and HADM, in which all modalities relevant to downstream tasks can be exhaustively covered. The proposed two-stage framework is shown in \ref{fig:model}, which will be introduced in details in the rest of this section.


%\xiaochen{A problem of the notation part: the data is too complex and hierarchical that cannot be easily represented through the subscript or superscript.}
\subsection{Problem Formulation}





Preprocessed inputs, regardless of modalities and levels, are transformed into sparse matrices, subject to feasible set denoted as $\mathbb{Z}_2 = \left\{0,1\right\}$. 
A patient can be represented by a sequence of Hospitalizations $H = \left\{h_1, h_2, ...,h_{|H|}\right\}$, where $\boldmath{|H|}$ denotes the number of Hospitalizations differing from patients. For each Hospitalization $h_n$, its corresponding diagnosis code is denoted as $D_n \in \mathbb{Z}_2^{|D|}$ where $|D|$ is the total of possible diagnosis codes. Pharmaceutical codes are represented as $P_n \in \mathbb{Z}_2^{|P|}$ where $|P|$ is the size of feasible set as well. $\boldmath{T_n}$ denotes the demographic table associated with $h_n$, whose dimension is denoted as $|T|$. Let $M_{n} = \left\{m_n^1, m_n^2, ...,m_n^{|M_{n}|}\right\}$ denotes sequence of ICU stay records associated with $h_n$, where $m_n^k \in \mathbb{Z}_2^{48 \times |m|}$ represents a 48 hours temporal record and $|m|$ is the feature amount of each time step, which is fixed across time steps, hospitalizations and patients. \ref{fig:data} shows the hierarchy of general EHR data. 


%A patient, denoted as $\textbf{p}$, can be represented by a sequence of HADMs $h_1, h_2, ...,h_{|H_p|} \in H$ , where $\boldmath{H_p}$ denotes the number of HADMs associated with this patient.

\subsection{Unimodal Encoding}

Regarding the heterogeneity across different modalities, we choose to adopt respective encoder responsible for generating unimodal representation based on modalities' characteristics. For temporal monitoring record represented as time series ($M_{n}$), Long Short Term Memory (LSTM) is adopted to generate its dense representation due to its capability of capturing unidirectional temporal information. Other modalities without any temporal factors are assigned with general multiple layer perceptron (MLP) serving as unimodal encoder. Setting unified dimension size of latent representation as $d_r$, latent representation of each modalities, denoted in the form of $R_{Modality}$, are generated as follow:

\xiaochen{Need to ask Boss Yin}
$$R_{m_n^k} = {LSTM}_{M}(m_n^k) | R_{T_n} = \text{ReLU}(\mathbf{W}_T T_n + \mathbf{b}_T) $$
$$R_{D_n} = \text{ReLU}(\mathbf{W}_D D_n + \mathbf{b}_D) | R_{P_n} = \text{ReLU}(\mathbf{W}_P P_n + \mathbf{b}_P)$$
%$$R_{T_n} = \text{ReLU}(\mathbf{W}_T T_n + \mathbf{b}_T)$$
%$$R_{D_n} = \text{ReLU}(\mathbf{W}_D D_n + \mathbf{b}_D)$$
%$$R_{P_n} = \text{ReLU}(\mathbf{W}_P P_n + \mathbf{b}_P)$$

%$$R_{m_n^k} = {LSTM}_{M}(m_n^k)$$
%$$R_{T_n} = {MLP}_{T}(T_n)$$
%$$R_{D_n} = {MLP}_{D}(D_n)$$
%$$R_{P_n} = {MLP}_{P}(P_n)$$

%where ${W}_T \in \mathbb{R}^{|T| \times d_r}$, ${W}_T \in \mathbb{R}^{|T| \times d_r}$, ${W}_T \in \mathbb{R}^{|T| \times d_r}$
\xiaochen{Too many matrices in different sizes, which will be listed in appendix}

\subsection{Multimodal Encoding}

After being passed through unimodal encoding, heterogeneous inputs from diverse modalities get unified to dense representation in the same size, which convent further aggregation. Transformer encoder has been widely recognized as a tremendous architecture able to fuse multiple modalities effectively. Different from popular fusion methods utilizing cross attention mechanisms, self attention receiving concatenation of multiple latent representations is adopted in this work, based on the consideration of the inconvenience of combining more than two modalities through cross attention.

Concerning that clinical time series is the only modality available in the level of ICU stay, its combination with diagnosis code and pharmaceutical code could be problematic, as these information are provided by the end of discharge, hinting their ambiguous temporal relation with each ICU stay and undermining the feasibility of this type of combination. On the contrast, the static nature of demographic table makes it an ideal modality injecting external information to clinical time series without any concerns about the alignment issue. Hence, we adopt demographic table as the background of patient, based on which model could make more comprehensive analysis on ICU stay simulating the decision-making process of medical practitioners.

After concatenation, the bimodal combination is delivered to a transformer encoder block in which self-attention is performed for modality fusion, followed by a linear layer compress the latent representation to the unified dimension size $d_r$.


$$R_{M_n^k}^{'} = Softmax(\frac{W_{M,q}[R_{m_n^k}, R_{T_n}] \cdot W_{M,k}[R_{m_n^k}, R_{T_n}]}{\sqrt{d_r}}) \cdot W_{M,v}[R_{m_n^k}, R_{T_n}]$$
$$R_{M_n^k} = W_d \cdot LayerNorm([R_{m_n^k}, R_{T_n}] + R_{M_n^k}^{'}) +b_d$$
%$$R_{M_n^k} = F_{M}([R_{m_n^k}, R_{T_n}])$$

as the representation of $k$ th Monitoring in $n$ th Hospitalization, where $[\cdot:\cdot]$ means the operation of concatenation, and $W_{M,q}, W_{M,k}, W_{M,v}, W_d \in \mathbb{R}^{d_r \times d_r}$, $b_d \in \mathbb{R}^{d_r}$.

To solve the alignment problem between admission and arbitrary Monitoring belonging to it, we design the following regulation mechanism: given the hyperparameter $l$ as the regularized length of $M_n$, we preserve first $l$ ICU stay for $M_n$ whose length is greater than or equal to $l$. For those whose length less than $l$, we pad the sequence with empty embedding $PAD$ whose length is $d_r$ as well. Thus, representation of all the Monitoring belonging to $H_n$ is obtained and denoted as $R_{M_n} \in \mathbb{R}^{l \times d_r} $.



%  \begin{align}
%    R_{M_n} = [ R_{M_n}^1,..., R_{M_n}^l] & \quad \textrm{if } |M_n| \geq l \\
%    R_{M_n} = [R_{M_n}^1 ... R_{M_n}^{|M_n|}, {PAD}^1, ...,{PAD}^{l-|M_n|}]                & \quad \textrm{if } |M_n| < l
%  \end{align}



According to Figure \ref{Fig.sub.1} and \ref{Fig.sub.2}, most of admissions possess less than 3 ICU stays, based on which we set the threshold $l$ to 3 in our experiments.


The fusion of modalities in the level of HADM is implemented based on the similar design, while the latent representation of modalities differ.

$$R_{H_n}^{'} = Softmax(\frac{W_{H,q}[R_{M_n}, R_{P_n}, R_{D_n}] \cdot W_{H,k}[R_{M_n}, R_{P_n}, R_{D_n}]}{\sqrt{d_r}}) \cdot W_{H,v}[R_{M_n}, R_{P_n}, R_{D_n}]$$
$$R_{H_n} = LayerNorm([R_{M_n}, R_{P_n}, R_{D_n}] + R_{H_n}^{'})$$

%$$R_{H_n} = F_{H}([R_{M_n}, R_{P_n}, R_{D_n}])$$
,where $W_{H,q}, W_{H,k}, W_{H,v} \in \mathbb{R}^{d_r \times d_r}$.
\subsection{Pretraining Tasks}

Given levelly-different representations $R_{M_n^k}$ and $R_{H_n}$, it becomes necessary to set appropriate target to enhance the quality of representation supervisely. Based on the analysis on hierarchical structure, we design one pretraining task concerning data reconstruction for ICU level, while two other pretraining tasks similar to masked language model (MLM) are assigned to HADM level.

\textbf{Clinical Time Series Reconstruction (CTSR).}  Given the representation of ICU stay $M_n$, the model is encouraged to reconstruct the clinical time series accordingly. This design follows the idea of autoencoder, which is widely adopted to obtain dense representation of time series. However, the reconstruction in \model is based on multimodal input that simulates the decision-making procedure in real world scenarios, targeting at the heterogeneity specially. 

A LSTM serving as decoder is responsible for the reconstruction:

$$ \hat{m}_n^k = LSTM_{CTSR}(R_{M_n^k})$$

followed by a Mean Squared Error (MSE) loss that usually serve in reconstruction tasks.

%$$ \mathbb{L}_{CTSR} = MSE(\hat{m}_n^k, {m_n^k})$$
$$ \mathbb{L}_{CTSR} = \frac{1}{n} \sum_{i=1}^n (\hat{m}_n^k - {m}_n^k)$$ 


\textbf{Masked Pharmaceutical Modeling (MPM).} Similar to MLM, in which tokens are randomly masked and expected to be predicted based on their context, MPM randomly masks pharmaceutical codes for each Hospitalization, while the definition of \textit{context} expanded: the model can not only retrieve the masked code using unmasked ones, but also rely on information from other modalities and other level. The prediction is implemented with a MLP block and the procedure is formed as follow:


$$ \hat{P}_n = Sigmoid(W_{MPM}R_{H_n} + b_{MPM})$$
%$$ \hat{P}_n = MLP_{MPM}(R_{H_n})$$

, where $W_{MPM} \in \mathbb{R}^{d_r \times |P|}$ and $b_{MPM} \in \mathbb{R}^{|P|}$. The predicted values serve as part of the MSE loss function:

%$$ \mathbb{L}_{MPM} = MSE(\hat{P}_n, {P}_n)$$
$$ \mathbb{L}_{MPM} = \frac{1}{n} \sum_{i=1}^n (\hat{P}_n - {P}_n)$$

\textbf{Masked Diagnosis Modeling (MDM).} The design of MDM is similar with MPM, while a separate MLP is responsible for predicting masked diagnosis codes:

$$ \hat{D}_n = Sigmoid(W_{MDM}R_{H_n} + b_{MDM})$$
%$$ \hat{D}_n = MLP_{MDM}(R_{H_n})$$ 

Parallelly, the MSE loss function is adopted for the supervision:

%$$ \mathbb{L}_{MDM} = MSE(\hat{D}_n, {D}_n)$$
$$ \mathbb{L}_{MDM} = \frac{1}{n} \sum_{i=1}^n (\hat{D}_n - {D}_n)$$
These two loss functions are jointly calculated as the final loss in the Hospitalization level pretraining without any weighting:

$$ \mathbb{L}_H = L_{MPM} + L_{MDM}$$






\subsection{Two Stage Hierarchical Pretraining}

 To advance the representation of different grannularies in EHRs, the two-stage pretraining strategy is adopted, optimizing $\mathbb{L}_{CTSR}$ and $\mathbb{L}_{H}$ respectively, in which a  high quality representation $R_{M_n}$ is initially obtained and benefits the optimization of $R_{H_n}$ subsequently. 






%\subsection{Pretraining on ICU Stay Level}

%Modalities associated with this level include clinical time series and demographic information represented in the tabular form. 

%Given the corresponding input pair from time series (${ts}_k$) and table (${tb}_k$), unimodal encoders specially designed for each modality will be utilized to obtain their unimodal representations:

%$$ R_k^{ts} = Encoder_{ts}({ts}_k) $$ 
%$$ R_k^{tb} = Encoder_{tb}({tb}_k) $$

%where in the implementation, the $Encoder_{ts}$ is a LSTM block while $Encoder_tb$ is in the form of MLP. Subsequently, these modality-specific representations are concatenated and sent to a self-attention block, such that mutual information from each modalities can be fully combined.

%$$ R_{icu} = Self\_Attn(Concat(R_k^{ts}, R_k^{tb})) $$

%For the sake of pretraining, we utilize the $R_{icu}$ to reproduce the ${ts}_k$ through the usage of a Decoder layer that is a LSTM in our implementation.

%$$ \hat{{ts}_k} = Decoder(R_{icu}) $$

%Thus, the pretraining loss in the ICU stay level is expressed as 

%$$ Loss_{icu} = Cross\_Entropy({ts}_k, \hat{{ts}_k})$$



%\subsection{Pretraining on HADM Level}

%Compared to the ICU stay level where only time series and table are available, more modalities can be utilized in the HADM level as many clinical actions are based on the unit of each visit, such as diagnosis and prescription, providing us with codes regarding diseases and drugs that can be regarded as a novel modality. In this level, we inherit the consequent we obtained from the ICU stay granularity, and aim at benefit downstream tasks in both levels.

%Similar to many typical complex data structures extracted from different databases or tables, the EHR data are connected in a highly complicated pattern. In the case of the relation between ICU stay and HADM, one can find from 0 to 7 ICU stays records given a specific HADM ID, which causes difficulties in the transferring learning between these two levels. For the simplicity and feasibility in the engineering perspective, we adopt the following algorithm to regulate the input form of our model in the HADM level:



%Given a HADM record $H$, denote the number of its corresponding ICU stays as $n$, then these ICU stays $R_H$ are represented as:


%  \begin{align}
%    R_H = \textrm{[} R_{icu}^1, ..., R_{icu}^l\textrm{]} & \quad \textrm{if } n \geq 3 \\
%    R_H = \textrm{[}R_{icu}^1 ... R_{icu}^|R_{icu}|, {[PAD]}^1, ...,{[PAD]}^1\textrm{]}                & \quad \textrm{if } n < 3
%  \end{align}
  
%, which means we only keep the first three time series for those HADMs possessing more than 3 ICU stays. Then the padding operation is conducted to ensure that the shape of $R_H$ is consistent regardless of the relation between HADM and ICU stays.







%\begin{itemize} 
%\item \textbf{Area Under the Receiver Operating Characteristic Curve (AUROC)}: 	

%\item \textbf{Area Under the Precision-Recall curve (AUPR)}:
%\end{itemize}





==> sections/related_works.tex <==
\section{Related Works}
Previous works have deeply explored the potential of applying typical pretraining strategies in multimodal scenarios, especially in the bimodal combination of vision and language \cite{luo_univl_2020, tan_vokenization_2020}. Similar with previous works in the monomodal setting \cite{cho_learning_2014, devlin_bert_2019}, these practices in multimodal domain also apply individual modules to encode information contained in each modality respectively. Based on the individual encoders, they further apply different strategies to combine representation leaned from different modalities by utilizing cross attention mechanism \cite{tan_lxmert_2019}, using approaches similar with self-attention mechanism after the concatenation of representations from different modalities \cite{chen_uniter_2020, ni_m3p_2021}, or even leveraging both of these strategies \cite{chen_visualgpt_2022, luo_univl_2020}. 
In these works, there are natural correspondences between modalities in the datasets. For instance, in the image captioning datasets used in some pretraining works \cite{chen_uniter_2020, pahde_multimodal_2021, socher_zero-shot_2013, tan_lxmert_2019}, the relationship between images and their corresponding textual description is explicit, making it easily for the deep learning model to learn the interaction across modalities. The same pattern can be observed in works regarding video captioning task \cite{huang_multimodal_2020} and video-audio matching circumstances \cite{liang_highmmt_2022}, in which a rough relation between video, audio and corresponding text can be captured and used as the guidance of deep neural network. 

Given the sort of correspondence mentioned above, two major types of pretraining strategies can be applied. The first one is MLM (masked language model) that has been named in accordance to its prevalent usage in pretraining in the field of natural language processing \cite{devlin_bert_2019}, referring to randomly masking some tokens in a sequence such that machine can learn from the relation between tokens through the reconstruction of the complete sequence. In the context of multimodal learning, this strategy can be leveraged in slightly different ways: the masking can be limited to a specific modality while information in other modalities is completely preserved \cite{huang_multimodal_2020, su_vl-bert_2021, tan_vokenization_2020}; also, random masking strategy can be simultaneously applied to multiple modalities \cite{geng_multimodal_2022, lu_vilbert_2019, shi_learning_2022}, urging models to exploit mutual information between modalities in a more effective way. Moreover, given other modalities serving as its context, one modality can be fully masked and the model is encouraged to reestablish the information from scratch \cite{shi_learning_2022}. These strategies do contradict to each other and can be leveraged jointly, with the use of addition in this final loss function.


The second category of pretraining strategies is predicting the alignment between data in pairs of modalities. An apparent instance is that given an image, the model is required to predict whether a piece of text is its corresponding caption, which can be regarded as a binary classification task as well. Nearly all the works mentioned above leverage alignment prediction along with their masking strategies, giving their model a higher capability of understanding the bidirectional relationships between different combinations of modalities. 

==> sections/related_works_new.tex <==
\section{Related Work} \label{related_works}




% \subsection{Multimodal Deep Learning}
% Multimodal deep learning, a subfield of deep learning emerging along with the work \cite{ngiam2011multimodal}, has becomes a popular topic after the success of several representative works in this area \cite{socher2013zero, frome2013devise, vinyals2015show, lu2019vilbert}. While the minority of these works pay attention to more than three modalities, most of them merely focus on the combination and interaction between two selected modalities and prove the learning cross different modalities can boost model's performance in diverse tasks. Following the design of some notable unimodal works\cite{cho_learning_2014, devlin_bert_2019}, recent practices in the multimodal domain choose to set encoder for each modality, and subsequently apply different strategies to perform modality fusion. Fusion strategies applied by these works can be briefly categorized into three types: 

% \begin{itemize}
%     \item \textbf{Simple combination}: The fusion is based on some simple mathematical operations on raw input or their latent representation such as addition, multiplication or averaging.\cite{zadeh_tensor_2017}
%     \item \textbf{Concatenation}: The fusion is performed through concatenation of raw input or their latent representation.\cite{chen_uniter_2020, ni_m3p_2021}
%     \item \textbf{Cross-modal DNN}: Multiple modalities are fused by utilizing DNN to perform the interaction between their latent representation. \cite{tan_lxmert_2019, chen_visualgpt_2022, luo_univl_2020, liang2018multimodal, perez2019mfas}
% \end{itemize}


% The simultaneous utilization of multiple modalities is based on the alignment between modalities. For instance, in works focusing on image captioning task \cite{chen_uniter_2020, pahde_multimodal_2021, socher_zero-shot_2013, tan_lxmert_2019}, the alignment between images and their corresponding textual description is explicitly defined, making it effortless for model to capture the interaction between modalities. The same pattern can be observed in works regarding video captioning task \cite{huang_multimodal_2020} and video-audio matching circumstances \cite{liang_highmmt_2022}. However, for complicated data structure such as EHR, alignment between modalities can be implicit or even ill-defined \cite{lee2023learning, zhang2022m3care}, complicating the multimodal learning.


% Given the sort of correspondence mentioned above, two major types of pretraining strategies can be applied. The first one is MLM (masked language model) that has been named in accordance to its prevalent usage in pretraining in the field of natural language processing \cite{devlin_bert_2019}, referring to randomly masking some tokens in a sequence such that machine can learn from the relation between tokens through the reconstruction of the complete sequence. In the context of multimodal learning, this strategy can be leveraged in slightly different ways: the masking can be limited to a specific modality while information in other modalities is completely preserved \cite{huang_multimodal_2020, su_vl-bert_2021, tan_vokenization_2020}; also, random masking strategy can be simultaneously applied to multiple modalities \cite{geng_multimodal_2022, lu_vilbert_2019, shi_learning_2022}, urging models to exploit mutual information between modalities in a more effective way. Moreover, given other modalities serving as its context, one modality can be fully masked and the model is encouraged to reestablish the information from scratch \cite{shi_learning_2022}. These strategies do contradict to each other and can be leveraged jointly, with the use of addition in this final loss function.


%The second category of pretraining strategies is predicting the alignment between data in pairs of modalities. An apparent instance is that given an image, the model is required to predict whether a piece of text is its corresponding caption, which can be regarded as a binary classification task as well. Nearly all the works mentioned above leverage alignment prediction along with their masking strategies, giving their model a higher capability of understanding the bidirectional relationships between different combinations of modalities. 

% \subsection{Pretraining for Electronic Health Records}

In recent years, researchers have extensively explored the applications of deep learning methodologies in the domain of healthcare, especially in the utilization of EHRs. Considering that labeled data is limited as annotation on EHRs demands domain knowledge and annotators professional skills \cite{chiu2017ehr, liang2019novel}, researchers turn to utilize pretraining technology to unsupervisely learning from EHRs datasets without any utilization of labels. 
\subsection{Unimodal Pretraining in Health Domain}




Regarding the heterogeneous nature of EHRs, most of researchers incline to develop their model on an unimodal basis. In recent years, Language Language Models (LLMs) have been witnessed to become successful in numerous domain regarding natural language processing, motivating researchers in the domain of health informatics pretrain their language model on clinical \cite{li2022clinical, lehman2023clinical, alsentzer2019publicly, peng2019transfer}, medical \cite{luo2022biogpt, lee2020biobert, yuan2022biobart, jin2019probing, warikoo2021lbert} and other scientific \cite{beltagy2019scibert} corpora to learn domain knowledge in this area. This sort of pretraining is in the admission-level, considering each admission respectively without any regards to other levels in the hierarchy of EHRs. 

Besides, other pretraining works \cite{rasmy2021med, li2020behrt, shang2019pre, choi2016multi, choi2018mime} turn to mine the information contained in structured codes. Similarly, this category of pretraining method aims at learning the representation of codes through the analysis on the patient level and fail to tackle more fine-grained tasks such as in ICU mortality prediction. 

\subsection{Multimodal Pretraining in Health Domain}

Multimodal pretraining is still a relatively understudied area in health-related domains. Previous works \cite{hervella2021self, hervella2022multimodal, hervella2022retinal, khare2021mmbert} aim at pretraining based on meidical image-text pairs, while minority of studies \cite{hager2023best} start pretraining using tabular information and image. Other work \cite{li2022hi} claiming their success on multimodal pretraining utilizes hand-crafted clinical features and diagnosis codes. However, these works only rely on two modalities, indicating the research gap that unification of more modalities avaialble in EHR is still absent.
